Using Convolutional Neural Networks to identify Gravitational Lenses in Astronomical images

The Euclid telescope, due for launch in 2021, will perform an imaging and slitless spectroscopy survey over half the sky, to map baryon wiggles and weak lensing. During the survey Euclid is expected to resolve 100,000 strong gravitational lens systems. This is ideal to find rare lens configurations, provided they can be identified reliably and on a reasonable timescale. For this reason we have developed a Convolutional Neural Network (CNN) that can be used to identify images containing lensing systems. CNNs have already been used for image and digit classification as well as being used in astronomy for star-galaxy classification. Here our CNN is trained and tested on Euclid-like and KiDS-like simulations from the Euclid Strong Lensing Group, successfully classifying 77% of lenses, with an area under the ROC curve of up to 0.96. Our CNN also attempts to classify the lenses in COSMOS HST F814W-band images. After convolution to the Euclid resolution, we find we can recover most systems that are identifiable by eye. The Python code is available on Github.

==> Bibliography.tex <==
\begin{thebibliography}{9}

%Test item
\bibitem{latexcompanion} 
Michel Goossens, Frank Mittelbach, and Alexander Samarin. 
\textit{The \LaTeX\ Companion}. 
Addison-Wesley, Reading, Massachusetts, 1993.

%Test item 
\bibitem{einstein} 
Albert Einstein. 
\textit{Zur Elektrodynamik bewegter K{\"o}rper}. (German) 
[\textit{On the electrodynamics of moving bodies}]. 
Annalen der Physik, 322(10):891–921, 1905.

%Test item 
\bibitem{knuthwebsite} 
Knuth: Computers and Typesetting,
\\\texttt{http://www-cs-faculty.stanford.edu/\~{}uno/abcde.html}

\bibitem{WalshDiscovery}
Walsh D., Carswell R. F., Weymann R. J., 1979, Nature, 279, 381

\end{thebibliography}

==> Conclusions.tex <==
\section{Conclusions}
5 lines arguing why neural networks are the correct way to go and what they have achieved already \\
20 lines on the current success, and why continued work in this area is important \\
5 lines on future development \\

==> Euclid_Strong_Lensing_Challenge.tex <==
\section{Euclid Strong Lensing Challenge}
10-20 lines on what the challenge was. \\
10-20 lines on my approach to the challenge \\
10-20 lines on the results of the challenge \\
Closing remarks on what has been learnt from the challenge. \\


==> Introduction.tex <==
\section{Introduction}
\medskip
The first strong gravitational lens system, QSO 0957+561, was recognised as such in 1979 when the spectra of two objects were compared and confirmed to be from the same object \cite{WalshDiscovery}. Gravitational lensing is caused by the mass of a foreground object, such as a galaxy or galaxy cluster, deflecting light from another distant source object, such as a galaxy or quasar. Strong gravitational lensing is rare with only a few expected from surveying thousands of objects (Blain 1996 and ). However lensing systems can be extremely useful cosmological tools. Lensed systems can be used to constrain the value of $h_{0}$, the Hubble constant, by measuring time delay (Refsdal 1964, Kochanek \& Schechter 2004), which occurs because the light from multiple images has taken different paths to reach the observer, introducing a time delay. Gravitational lensing is independent of the lensing object's luminosity and depends only on the mass of the lens object and the geometry of the source and the lens relative to the observer. This makes lensing a unique tool for analysing mass distribution in the foreground lens (Treu \& Koopmans 2002). Using this dependence on mass alone, and combining mass models from mass-luminosity analysis, the baryonic and dark matter mass of the galaxy can be mapped to find dark matter substructure (Vegetti et al. 2012, Metcalf \& Madau 2001). Gravitational lensing conserves surface brightness but not the size of the source object, causing an effective magnification of the source object's flux, if the image of the source is enlarged. This enables the observation of fainter galaxies which would otherwise be missed, including galaxies at high-redshifts  (Claeskens et al. 2006, Jackson 2011).
\par
Currently the Sloan Lens ACS Survey (SLACS) has provided the most strong lensed systems from a single survey, with nearly 100 observed (Bolton et al. 2008). Other sources of strong lenses include the Kilo-Degree Survey (KiDS) (de Jong et al. 2015) which uses the VLT Survey Telescope at the Paranal Observatory in Chile, the Dark Energy Survey (The Dark Energy Survey Collaboration 2005), the Subaru Hyper Suprime-Cam Survey (Miyazaki et al. 2015), these current optical wide surveys, expected to observed thousands of lenses (Collett 2015). Jodrell Bank–Very Large Array (VLA) Astrometric Survey (JVAS; Patnaik et al. 1992; Browne et al. 1998; Wilkinson et al.
1998) and the Cosmic Lens All-Sky Survey (CLASS; Browne et al. 2003; Myers et al. 2003) have detected 22 radio loud lensed active galactic nuclei (Chae et al. 2002). 
\par
Future telescopes are expected to observe many more strongly lensed systems , the Euclid telescope (Laureijs et al. 2011) and the Large Synoptic Survey Telescope (LSST Science Collaboration et al. 2009), will bring the total number of systems above $10^{5}$(Oguri \& Marshall 2010, Collett 2015, Serjeant 2016). Euclid will map three-quarters of the extragalactic sky with Hubble Space Telescope resolution (quote) to 24 magnitude (Amendola et al. 2013). Another project, the Square Kilometer Array (Rawlings \& Schilizzi), will take observations at a  resolution of 2 mas at 10 GHz, and 20 mas at 1 GHz (Dewdney et al. 2009; Godfrey et al. 2012), and is expected to observe a similar figure to the new telescopes. 
\par
There is currently a shift in the methodology for detecting strongly lensed systems in astrophysical images as sample sizes of lens candidates becomes much larger. Traditionally most images were found by eye, 112 lens candidates, and at least 2 certain lenses, were found in a HST legacy programme, looking at the COSMOS field (Faure et al. 2008, Jackson 2008). But not all searching by eye has been carried out by people working in strong gravitational lensing, the public have been tasking with finding new lens candidates using Space Warps (Marshall et al. 2016). Space Warps makes use of citizen science and crowd sourcing to have volunteers analyse a large number of images by eye to look for lensing features, via an online webpage similar in execution to that of Galaxy Zoo (Willett et al. 2013). Tens of new lens candidate have been identified from these volunteers, using large ground-based surveys, e.g. the Canada-France-Hawaii Telescope Legacy Survey (More et al. 2016). But with the growth of survey size, candidate detection on the levels of the Space Warps project is not high enough to satisfy the large number expected from the future surveys. There have been several successful methods of computational searches for lenses. Arcfinder (Seidel \& Bartelmann 2007) uses pixel-grouping methods to attempt to find cluster-scale lens systems, Ringfinder (Gavazzi et al. 2014) searches for blue residuals surrounding early-type galaxies using multi-band data, and there are several programs to find arc-like shapes (Lenzen et al. 2004, More et al. 2012). In recent years there has been a rise in machine-learning methods to detects lenses. 56 lens candidates were found in the KiDS dataset by using a convolutional neural network (Petrillo et al. 2017). Machine learning methods rely on large datasets in order to train and learn, something which has become available in recent years. Once a machine has been trained, the fast classification of images is very easy and exactly what is required as more data becomes available. 




 Also the sources are bright at submillimeter wavelengths, making them easier to detect whilst being obscurred by the foreground lens. 
To constrain the equation of state of dark matter, w, rare lens systems with a double source plane must be observed and analysed. 




\begin{thebibliography}{9}

%Test item
\bibitem{latexcompanion} 
Michel Goossens, Frank Mittelbach, and Alexander Samarin. 
\textit{The \LaTeX\ Companion}. 
Addison-Wesley, Reading, Massachusetts, 1993.

%Test item 
\bibitem{einstein} 
Albert Einstein. 
\textit{Zur Elektrodynamik bewegter K{\"o}rper}. (German) 
[\textit{On the electrodynamics of moving bodies}]. 
Annalen der Physik, 322(10):891–921, 1905.

%Test item 
\bibitem{knuthwebsite} 
Knuth: Computers and Typesetting,
\\\texttt{http://www-cs-faculty.stanford.edu/\~{}uno/abcde.html}

\bibitem{WalshDiscovery}
Walsh D., Carswell R. F., Weymann R. J., 1979, Nature, 279, 381

\end{thebibliography}

==> Limitations_of_the_Neural_Network.tex <==
\section{Limitations of the Neural Network}

==> Neural_Networks.tex <==
\section{Neural Networks}
\medskip
Neural Networks (NNs) are built from individual artificial neurons called perceptrons. A perceptron is designed to simulate the role of a biological neuron, but with the advantage that a mathematical function can be used for activation of the neuron \cite{Aggarwal}. Layers in a NN are built from a number of perceptrons which all use outputs from perceptrons in the previous layer. A perceptron takes a number of inputs, applies a weight to each, sums these products, applies a bias, and then is used as input to an activation function, which then gives the perceptrons output. If we let $\textbf{x}$ be the 1-d vector of inputs, $\textbf{y}$ be the 1-d vector of weights associated with this perceptron, $b$ be the bias, and $f$ be the activation function, then the output $z$ is calculated using: 
\begin{equation}
z = f(\sum_{n=1}^{k} x_{i} y_{i}  + b)
\end{equation} 
where $k$ is the number of inputs to the perceptron. The function $f$ is kept the same for each perceptron in a single layer, but can differ in different layers of the network to improve performance. For a binary classification problem a sigmoid function is often used. The output $z$ from the perceptron is then used as input for the perceptrons in the next layer of the network. In a fully-connected layer, all the outputs from the previous layer are used as the input for all the perceptrons in the current layer. 
\par
Neural networks have to be trained before they can be used for classification problems, through a process of supervised or unsupervised learning. Supervised learning means that the data used to train the network has already been labelled with the correct classification for each object, whereas in unsupervised learning, no label of classification is given. Once the network has been trained, new unseen data can be classified by the network, with the classification resulting from what the network has learned from in the training phase. During the training phase, weights and biases from each neuron are altered as the network learns. They are altered through stochastic gradient descent, a method of changing the weights and biases in the correct direction in order to improve the classification, and learn to find patterns. More complicated structures called Convolutional Neural Networks (CNNs) are often used to find features and patterns in images. Layers in a NN made from just perceptrons are called dense layers.  
\par
CNNs are a subset of NNs which use convolution layers in the network for image recognition or classification. A convolution layer involves a kernel being convolved with an input image in order to make a feature map. Often the convolution layer has several different kernels for the same image, meaning several different feature maps are given as output. The image kernel can either be pre-determined, or can be another parameter that the network trains and improves. Different layers may have different image kernel sizes, as well as different sized image outputs. Between convolution layers, pooling layers are often integrated. A pooling layer is designed to greatly reduce the pixels in an input image to speed up training and reduce the number of parameters. Pooling is generally done one of two ways, max pooling or mean pooling. Both methods look at a small section of the image, say a 2 x 2 section, and reduces this to one pixel value by either finding the maximum value in the 2 x 2 sqare or by finding the mean. The output is then a reduced image with 4 times fewer pixels than the original output. Pooling is done to reduce the variables whilst trying to keep as much spacial information in the image as possible [Ref]. The convolution layers in a CNN are designed to process visual information hierarchically, with earlier layers finding more basic features, and later layers building on what layers before have found to build up more complicated features within the image. This is how the network can go from seeing individual pixel values to finding complicated features, such as a face. Each layers filters the input image in a different way to create feature maps which work as the input for the next layer. Often an image filtering layer will make use of several kernels which in turn makes several feature maps from the same input image. After the convolution and pooling layers, the pixels from the feature maps of the final convolution or pooling layer is then flattened into a 1-d vector with a flattening layer. This 1-d vector can then be used as input for a NN made from dense layers of perceptrons. One of the first neural networks designed to work like this was the Neocognitron in 1980 \cite{Fukushima}. In Convolutional neural networks, the weights for each of the kernels are not fixed, and are initialised randomly. These weights are then changed in a supervised way in order to improve the performance of the network \cite{Ciresan}. 
\par
The MNIST database is a collection of 70,000 images of handwritten digits, ideal for testing pattern recognition and classification programs. There have been hundreds of attempts over the past 20 years, using various methods, to get the error rate as low as possible. The error rate is the percentage of digits the program incorrectly classifies. Currently the best attempts to classify all the digits correctly has been using neural networks, more specifically convolutional neural networks, where the error rate has decreased to 0.23 (Ciresan et al. CVPR 2012). Add more and mention the CIFAR-10 image classification problem
%http://yann.lecun.com/exdb/mnist/

\begin{thebibliography}{9}

\bibitem{Fukushima}
Kunihiko Fukushima. Neocognitron: A
self-organizing neural network for a mechanism of pattern
recognition unaffected by shift in position. Biological Cybernetics,
36(4):193–202, 1980.

\bibitem{Ciresan}
Ciresan, D. C., Meier, U., Masci, J., Gambardella, L. M., and Schmidhuber, J. Flexible, high performance
convolutional neural networks for image classification. In IJCAI, pp. 1237–1242, 2011.

\bibitem{Aggarwal}
Aggarwal C. C., 2014, Data classification: algorithms and applications. CRC Press.

\end{thebibliography}

==> Training_the_Neural_Network.tex <==
\section{Training the Neural Network}
10 lines on implementation within python \\
20 lines on training the network \\
20 lines on network architectures and various changes made \\
20 lines showing continued improvements, and the finished results \\
